Capturing Perspectives of Crowdsourced Annotators in Subjective Learning Tasks

Supervised classification heavily depends on datasets annotated by humans. However, in subjective tasks such as toxicity classification, these annotations often exhibit low agreement among raters. Annotations have commonly been aggregated by employing methods like majority voting to determine a single ground truth label. In subjective tasks, aggregating labels will result in biased labeling and, consequently, biased models that can overlook minority opinions. Previous studies have shed light on the pitfalls of label aggregation and have introduced a handful of practical approaches to tackle this issue. Recently proposed multi-annotator models, which predict labels individually per annotator, are vulnerable to under-determination for annotators with few samples. This problem is exacerbated in crowdsourced datasets. In this work, we propose \textbf{Annotator Aware Representations for Texts (AART)} for subjective classification tasks. Our approach involves learning representations of annotators, allowing for exploration of annotation behaviors. We show the improvement of our method on metrics that assess the performance on capturing individual annotators' perspectives. Additionally, we demonstrate fairness metrics to evaluate our model's equability of performance for marginalized annotators compared to others.

==> temp_writings/more_exp_ideas.tex <==
\section{More experiment ideas}

\subsection{Adding synthetic annotators}
We make some synthetic data! 

\paragraph{Method 1}
let's add two fake annotators. 
One of them always predicts the maj vote and the other always predicts the opposite! 
Train the three models on the data! 

Do the models predict correct label for those two labels? (what is personalized F1 for those two annotators?

After Training AART look at the embeddings of those two! where do they fall in the space? 


\paragraph{Other Methods}
other methods can include having more of maj-vote guy and more of always-opposite guy and assign them to $20\%$ of data! 



Practical questions! 
1) which data to start with? 
I would say Maarten Sap datasets 

2) how to split? 

3) do I have to pretrain on another dataset first? (because Maarten Sap's data is small) 

4) can I have my fake annotators representing liberals vs conservatives? 

Micro steps:
I will add the fake annotators
With 5 different random seeds I will split to train dev and test, each time I will try for different hyper parameter parameters based on train, will choose the best HP comb based on dev. and then will calculate evaluation metrics on test sets. 

How single-task will fail? because it probably will have the same prediction for both fake annotator #1 and fake annotator #2 (unless it always give 50-50 probabilites for 0 and 1? 

\subsection{Demographic groups}
\subsubsection{The experiments we were doing about adding up demographic embeddings to the annotator embeddings}
refer to slides for them, I think the idea was neat! 
\subsubsection{Zhivar's suggestion about pretraining annotator embeddings using demographics}
At first don't designate a separate embedding for each annotator but only have a separate embedding for each demographic treat. After training the model in that setting then initialize each annotator's embedding with its demographic embedding. 
\paragraph{Details!} what if there are several demographic features available? Then for each combination we can designate a separate embedding e.g. <white, woman>, <white, man>, <black, woman>, <black, man> 

\subsection{Noise and uncertainty}
Can we add a few fake noisy annotators and analyze the below hypothesis? Do the following metrics show those fake noisy annotators are actually very noisy? Do the following metrics by mistake consider the minority annotators as noisy (for example black people)?

What happens if we remove the annotators considered as noisy (by the following metrics) and train AART/multi-task again? Also test on new out of domain data to see if the performance decreases/increases there. 
\subsubsection{recognizing noisy annotators from standard-deviation}
If we repeat the training of AART/multi-task for several random seeds, can we say the annotators that show a very high standard deviation in their F1 are noisy? 

\subsubsection{recognizing noisy annotators from data maps confidence}
The work we are doing with the kids can include this


\subsection{New annotators in test?}
Fred: let's consider new annotators in test or in general out of domain samples in test (that also have new annotators)

Myrl and Valerio both have suggested seeing a new annotator in test with a few samples from it. Can we do a few shot learning and expand our model to that annotator?
Myrl suggests averaging up embeddings of some previously seen similar annotators to estimate an embedding for the new annotator 


\subsection{Kian suggested a new architecture}
He was suggesting freezing bert and adding a few feed-forward layers on top of it. 
